Robust Path Recommendations During Public Transit Disruptions Under Demand Uncertainty

When there are significant service disruptions in public transit systems, passengers usually need guidance to find alternative paths. This paper proposes a path recommendation model to mitigate congestion during public transit disruptions. Passengers with different origins, destinations, and departure times are recommended with different paths such that the system travel time is minimized. We model the path recommendation problem as an optimal flow problem with uncertain demand information. To tackle the lack of analytical formulation of travel times due to capacity constraints, we propose a simulation-based first-order approximation to transform the original problem into a linear program. Uncertainties in demand are modeled using robust optimization to protect the path recommendation strategies against inaccurate estimates. A real-world rail disruption scenario in the Chicago Transit Authority (CTA) system is used as a case study. Results show that even without considering uncertainty, the nominal model can reduce the system travel time by 9.1% (compared to the status quo), and outperforms the benchmark capacity-based path recommendation. The average travel time of passengers in the incident line (i.e., passengers receiving recommendations) is reduced more (-20.6% compared to the status quo). After incorporating the demand uncertainty, the robust model can further reduce system travel times. The best robust model can decrease the average travel time of incident-line passengers by 2.91% compared to the nominal model. The improvement of robust models is more prominent when the actual demand pattern is close to the worst-case demand.

==> record_some_formula <==

% And the corresponding robust counterpart is

% 
% \begin{align}
%      (\boldsymbol{A} \bar{\boldsymbol{d}})^T \boldsymbol{p} + \rho_{1-\varepsilon}  \norm{(\boldsymbol{AD})^T\boldsymbol{p}}_2 \leq b
%      \label{cont_RC}
% \end{align}
 


% \begin{align}
% \max_{\boldsymbol{d} \in \mathcal{D}}  \min_{\boldsymbol{f} \in \mathcal{F}(\boldsymbol{d})}  Z(\Tilde{\boldsymbol{f}}) + \boldsymbol{\beta}(\Tilde{\boldsymbol{f}})^T (\boldsymbol{f} - \Tilde{\boldsymbol{f}})
% \end{align}



% \subsection{Incident duration uncertainty}




% Calculation of . 

% Intro to network loading here:

% Run a network loading model based on $\Tilde{\boldsymbol{f}}$. Then we know $Z({\boldsymbol{\Tilde{\boldsymbol{f}}}})$. Question is how to get $Z({\Tilde{\boldsymbol{f}} + \boldsymbol{e}_{hkr}})$ without processing the network loading. 

% $q_i \in Q_{hkr}$ is the set of all queues of the $i$-th boarding platform of path $r$ for $f_{hkr}$ (exist passengers in $M_{hkr}$ in these queues, queue are defined as a group of waiting passengers at the time when a vehicle arrival).

% Set of vehicles $v \in V_{hkr}$.


% sum over segment index (TO BE DONE)

% \begin{align}
% Z({\Tilde{\boldsymbol{f}} + \boldsymbol{e}_{hkr}}) - Z({\boldsymbol{\Tilde{\boldsymbol{f}}}}) \approx \frac{\sum_q t_q}{|Q_{hkr}|} + \frac{\sum_v t_v^{\text{wait}} + t_v^{\text{in-veh}}}{|V_{hkr}|}
% \end{align}




% There are several uncertainties in the system: 1) the duration of the disruption is a random variable that can be modeled as a discrete variable (e.g., 30 min, 40 min, 50 min, etc). 2) the travel demand $d_{hk}$ is a random variable, which can be modeled as a joint Gaussian distribution. 3) After obtaining the optimal flow $f_{hkr}^*$, we need to figure out the recommendation strategy to each passenger in $d_{hk}$ such that the final flows are as close to $f_{hkr}^*$ as possible. Given behavior uncertainty, a passenger $p$ may only follow the recommendation with probability $\alpha_p$. 

% The disruption duration uncertainty can be modeled as a SO (i.e, the objective function is modeled as the expectation over all possible duration scenarios). \textbf{The demand uncertainty can be modeled by RO with an ellipsoidal uncertainty set. The mean and covariance matrix of $d_{hk}$ can be estimated from smart card data (available in our lab)}. The behavior uncertainty is addressed separately in another optimization problem. In this problem, we only need to provide an upper and lower bound for $f_{hkr}$ to represent the range of the number of passengers that will follow the path recommendation. 


% \subsection{Passenger behavior uncertainty}
% Consider passenger behavior uncertainty that they may not follow the recommendations. Then $\boldsymbol{f}$ is random variable. However, the optimization model cannot directly solve for random decision variables. The typical way is to solve moments or distribution parameters of the random decision variables \citep{hernandez2018introduction}. Hence, with a slight abuse of notations, assume that in the optimization model,  $\boldsymbol{f}$ represents the expectation of path flows and $\boldsymbol{p}$ the expectation of path shares. The behavior uncertainty actually provides a lower and upper bound for the expectation. For example, if we recommend all $d_{hk}$ to (resp. not to) use path $r$, then $f_{hkr}$ reaches the upper (resp. lower) bound. $f_{hkr}$ within the lower and upper bounds are the expected flows that can be realized even if there is non-compliance behavior. 

% Assume that all passengers have some intended (original) path choices if no recommendation is provided. And let $q_{hkr}$ be the intended path shares for path $r \in R_k$. If passengers did not follow the recommendation, they would use the their intended paths. Define $\alpha_{hkr,r'}$ as the probability that passengers with intended path choice of $r'$ following the recommendation of using path $r$. $\alpha_{hkr,r} = 1$ and $\alpha_{hkr,r'}$ ($r' \neq r$) is some pre-determined constant. Considering that not all passengers will use the path recommendation system due to reasons such that lack of access or being confident about their intended path, we defined $\mu^{\text{N}}_{hk}$ as the proportion of passengers not using the recommendation system (referred to as non-accessible passengers), and $\mu^{\text{A}}_{hk} = 1 - \mu^{\text{N}}_{hk}$ is the proportion of passengers using the recommendation system (referred to as accessible passengers). Then for a given OD pair $k$ and time $h$, the lower bound of the path share expectation $p_{hkr}$ happens when all accessible passengers are recommended to ``not'' use path $r$:

% 
% \begin{align}
%  p_{hkr} \geq \mu^{\text{N}}_{hk} \cdot q_{hkr} + \mu^{\text{A}}_{hk} \cdot q_{hkr} \cdot (1-\max_{r'\in R_k \setminus\{r\}}\alpha_{hkr',r})  \quad \forall (h, k, r) \in \mathcal{F}
%  \label{eq_lower_p}
% \end{align}
% The first term represents the proportion of passengers who do not use the recommendation system and originally intend to use path $r$. And the second term represents the proportion of passengers who intend to use path $r$ and are recommended not to use path $r$, but do not follow the recommendation (i.e., they still use path $r$). The ``$1-\max_{r'\in R_k \setminus\{r\}}\alpha_{hkr',r}$'' term represents passengers are recommended with a path $r' \neq r$ that they are most likely to follow (so that $p_{hkr}$ reaches the lower bound). 
% Note that an implicit assumption in Eq.  \ref{eq_lower_p} is that using the recommendation system or not is independent of their intended path choice behavior. This assumption can be easily relaxed by changing $\mu^{\text{A}}_{hk} \cdot q_{hkr}$ to a joint probability term meaning the proportion of accessible passengers with intended path $r$. 

% Similarly, the upper bound for the path share expectation happens when all accessible passengers are recommended to use path $r$:

% 
% \begin{align}
%  p_{hkr} \leq \mu^{\text{N}}_{hk} \cdot q_{hkr} + \mu^{\text{A}}_{hk} \cdot q_{hkr}+  \mu^{\text{A}}_{hk}  \sum_{r' \in R_k \setminus\{r\}} \alpha_{hkr,r'} \cdot q_{hkr'}  \quad   \forall (h, k, r) \in \mathcal{F}
%  \label{eq_upper_p}
% \end{align}
% The second term in Eq. \ref{eq_upper_p} represents the proportion of passengers whose intended path is $r$ and they are recommended to use path $r$. In this case, all of them will follow the recommendation. The third term in Eq. \ref{eq_upper_p} means the proportion of passengers whose intended path is not $r$ and they are recommended to use path $r$ and follow the recommendation.

% For any $p_{hkr}$ exceeding the lower or upper bound, the path share expectation cannot be reached by any strategies of recommendation given the ``non-compliance'' of passengers. The definition of the lower and upper bound is to ensure that after solving the ``optimal path shares'', we can make the final expected passenger flows reach this path shares using some recommendation strategies (details in Section \ref{sec_recommend}). 

% However, given imperfect passenger behavior model, $\mu^{\text{A}}_{hk}$ and $q_{hkr}$ may be unavailable or include uncertainties. In this study, we assume $\mu^{\text{A}}_{hk}$ are known constants and we only consider the uncertainty in $q_{hkr}$. The reasons are as follows: 1) operators can usually collect passenger preference of using the recommendation system (i.e., $\mu^{\text{A}}_{hk}$) in advance with a simple ``Yes/No'' question. 2) Considering the multiplication of two uncertain variables is usually challenging. 


% Consider a polyheron uncertainty set for $q_{hkr}$:

% 
% \begin{align}
%     \mathcal{Q} = \left\{\boldsymbol{q}\in \mathbb{R}^{|\mathcal{F}|}: \sum_{r\in R_{k}} q_{hkr} = 1,  q_{hkr} \in [ \bar{q}_{hkr} - \gamma_{hkr},\bar{q}_{hkr} + \gamma_{hkr}] , \forall (h, k, r) \in \mathcal{F} \right\}
% \end{align}
% where $\boldsymbol{q} = (q_{hkr})_{h,k,r \in \mathcal{F}}$, $\bar{q}_{hkr}$ is the nominal value of ${q}_{hkr}$ and $\gamma_{hkr}$ is the parameter of uncertainty range which satisfy $\bar{q}_{hkr} - \gamma_{hkr} \geq 0$ and $\bar{q}_{hkr} + \gamma_{hkr} \leq 1 \; \forall (h,k,r) \in \mathcal{F}$. Both values can be obtained from survey or empirical studies \citep{rahimi2020analysis,mo2021inferring}. And the robust counterpart for Eq. \ref{eq_lower_p} and \ref{eq_upper_p} is:

% 
% \begin{align}
% p_{hkr}^{\text{L}} \leq p_{hkr} \leq p_{hkr}^{\text{U}} \quad  \forall (h, k, r) \in \mathcal{F}
% \end{align}
% where $p_{hkr}^{\text{L}} = (1-\mu^{\text{A}}_{hk}\alpha_{hkr} )\cdot(\bar{q}_{hkr} + \gamma_{hkr})$ and $p_{hkr}^{\text{U}} =  \sum_{i=1}^{|R_k|} \hat{q}_{hkr_i}$, $\hat{q}_{hkr_i} = \min\{\bar{q}_{hkr_i} + \gamma_{hkr_i}, 1 - \sum_{j=1}^{i-1} \hat{q}_{hkr_j}\}$. Here we name the path ID as $r_1,...r_{|R_k|}$ st. $w_{hkr_i} \leq w_{hkr_j}...$ for all $i \leq j$, where $w_{hkr_i} = \mu_{hk}^{\text{A}}\alpha_{hkr_i}$ if $i \neq |R_k|$, and $w_{hkr_{|R_k|}} = 1$. 

% Due to the limit of space, we omit the derivation of the robust counterpart. The basic idea of the upper bound derivation is to assign the highest share to smallest-weight $q_{hkr}$ so as to get the minimum.  

% %(note that $r_{n_k} = r$ because $w_{hkr} = 1$ is the largest weight)

% \begin{align}
% p_{hkr}^{\text{L}} =(1-\mu^{\text{A}}_{hk}\alpha_{hkr} )\cdot(\min\{1,\bar{q}_{hkr} + \gamma_{hkr}\})
% \end{align}


% \begin{align}
%     f^{\text{N}}_{hkr} = d_{hk} \cdot \mu^{\text{N}}_{hk} \cdot q_{hkr}\\ 
%     f^{\text{A}}_{hkr} = d_{hk} \cdot \mu^{\text{A}}_{hk} \cdot q_{hkr}
% \end{align}
% where $ \mu^{\text{N}}_{hk} +  \mu^{\text{A}}_{hk} = 1$,  $\sum_{r \in R_k} q_{hkr} = 1$. $q_{hkr}$ is also uncertain. It is estimated from some previous model.

% To calculate the corresponding bounds, 

% % consider $M_{hk}$. Number of passengers intended to use $r$ and not asking for suggestions. $f^{\text{U}}_{hkr}$. $f_{hkr}^{\text{A}}$ passengers intended to use $r$ and but asking for suggestions.

% aggregate probability . (can be individual level: for future research)



% Find the min bounds for the expectation. Recommend all passengers we can reach not using $r$, lower bound:

% \begin{align}
% {f}_{hkr}^{\text{L}} = f^{\text{N}}_{hkr} + (1-\alpha_{hkr}) f_{hkr}^{\text{A}} 
% \end{align}

% Upper bound: recommend all passengers using path $r$

% \begin{align}
% {f}_{hkr}^{\text{U}} = f^{\text{N}}_{hkr} + f_{hkr}^{\text{A}} + \sum_{r' \neq r} \alpha_{hkr'} f_{hkr'}^{\text{A}}
% \end{align}


% A set of passengers whose intended path is $r$:  


% With slight abuse of notation, we assume in the optimal flow stage, $f$ represents the expectation of flows.

% constraints of $f_{hkr}$:
% \begin{align}
% {f}_{hkr}^{\text{L}} \leq f_{hkr} \leq {f}_{hkr}^{\text{U}} \ \quad \forall h, k, r 
% \end{align}

% Divided by $d_{hk}$ and write it regarding $p_{hkr}$:

% \begin{align}
%  p_{hkr} \leq q_{hkr} +  \mu^{\text{A}}_{hk}  \sum_{r' \neq r} \alpha_{hkr'} \cdot q_{hkr'} \ \quad \forall h, k, r
% \end{align}


% Define
% \begin{align}
%     \mathcal{F}(\boldsymbol{d}) = \{\boldsymbol{f}: \sum_{r\in R_{k}} f_{hkr} = d_{hk},  {f}_{hkr}^{\text{L}}(d_{hk}) \leq f_{hkr} \leq {f}_{hkr}^{\text{U}}(d_{hk}), {f}_{hkr} \geq 0, \forall h, k, r\}
% \end{align}


% RC:
% \begin{align}
%  p_{hkr} \leq q_{hkr} +  \mu^{\text{A}}_{hk}  \sum_{r' \neq r} \alpha_{hkr'} \cdot q_{hkr'} \ \quad \forall \boldsymbol{q}\in \mathcal{Q}, \forall h, k, r
% \end{align}

% \begin{align}
%  p_{hkr} \leq \min_{\boldsymbol{q}\in \mathcal{Q}}( q_{hkr} +  \mu^{\text{A}}_{hk}  \sum_{r' \neq r} \alpha_{hkr'} \cdot q_{hkr'})  \ \quad \forall h, k, r
% \end{align}



% Given the uncertainty set of $\mathcal{Q}$, this is equivalent to a simple assignment problem. weight of $q_{hkr}$ is 1, and the weight of $q_{hkr'}$ ($r'\neq r$) is $\mu^{\text{A}}_{hk}\alpha_{hkr'} \leq 1$. Total resource is 1. Assign to the smallest weight first. 

% Define weight: $w_{hkr'} = 1 $ or 

% \begin{align}
%     \min_{\boldsymbol{q}\in \mathcal{Q}}( q_{hkr} +  \mu^{\text{A}}_{hk}  \sum_{r' \neq r} \alpha_{hkr'} \cdot q_{hkr'}) = \bar{q}_{hkr} + \gamma_{hkr}
% \end{align}

% WLOG. let $r_1,...r_{n_k}$ st. $w_{hkr_i} \leq w_{hkr_j}...$ for all $i \leq j$ (note that $r_{n_k} = r$ because $w_{hkr} = 1$ is the largest weight)

% $q^*_{hkr_i} = \min\{\bar{q}_{hkr_i} + \delta_{hkr_i}, 1 - \sum_{j=1}^{i-1} q^*_{hkr_j}\}$

% Denote it as $p_{hkr}^{\text{U}} = \sum_{i=1}^{n_k} q^*_{hkr_i}$

% Similarly:
% we have 
% \begin{align}
%  p_{hkr} \geq q_{hkr} - \alpha_{hkr} \cdot \mu^{\text{A}}_{hk} \cdot q_{hkr}  \ \quad \forall \boldsymbol{q}\in \mathcal{Q}, \forall h, k, r
% \end{align}
% \begin{align}
%  p_{hkr} \geq \max_{\boldsymbol{q}\in \mathcal{Q}} (q_{hkr} - \alpha_{hkr} \cdot \mu^{\text{A}}_{hk} \cdot q_{hkr})  \ \quad \forall h, k, r
% \end{align}



% Future study may consider sacrificing some of the closeness of the expectation to reduce the variation in the system. 

% This can be formulated as solving a system of linear equations:

% 
% \begin{align}
%     p_{hkr}^* = \mu_{hk}^U \cdot q_{hkr} + \mu_{hk}^A\left[q_{hkr} \sum_{r'\in R_k \setminus \{r\}}s_{hkr'}(1-\alpha_{hkr'}) + s_{hkr}\sum_{r'\in R_k \setminus \{r\}} q_{hkr'}\cdot \alpha_{hkr'} \right], \quad \forall (h,k,r) \in \mathcal{F}
% \end{align}
% The first term means the proportion of passengers that do not use the recommendation system and their original choice is path $r$. The second term represents the proportion of passengers using the system, with original choice of path $r$, getting the recommendation to use $r'\neq r$ but not following the recommendation. And the third term indicates the proportion of passengers using the system, with original choice of path $r' \neq r$, getting the recommendation to use $r$ and following the recommendation.

% $s_{hkr}$ can be obtained by solving the system of linear equations (for a specific $(h,k)$, there are $|R_k|$ independent equations and $|R_k|$ unknown variables). And it can be easily verified that the solved $s_{hkr}$ satisfying $\sum_{r\in R_k} s_{hkr}= 1$.

% Another way to understand: match to probability. indicator variable E(1(choice = r)) = p(choice = r) = p available*p original choice + p not available... .... 

% Variance. p hkr star. (every passenger is the same, homogeneous). 


% \subsection{Preliminaries}
% two types of network loading: frequency-based and dynamic based, frequency-based static, not suitable for incident control as the frequency may change over time. Use schedule-based. Input: path flows. Path includes all transfer patterns, no common line problems. Event-based Network loading process. Why travel time no analytical formulation: waiting time: available capacity, how many passengers board before, previous boarding determined by their previous boarding, and so on. How many transfer passengers, transfer passengers determined by when they can board the first segment. 




% Get worst-case demand:



% \subsection{Solution algorithm}
% Step 1: initial demand (e.g., d nominal). initial path share, run simulation get beta.

% Step 2: 

% MSA: Convergence criteria:

% This is not a continuous problem, the fixed point may not exist. in fact, $\beta_{hkr}$ in two successive iterations can be arbitrarily large. We define a fixed region. average $Z(f)$ of last $K$ iterations. if $|Z(f)^{(k)} - Zf| < \epsilon$, stop. Intuition, though not continuous, the $Z_f$ change when it is close to optimal should be within a range. Take the best $k$ over the last $K$ as the final solution.

% \subsection{Recommendation strategy}\label{sec_recommend}
% Let $\boldsymbol{p}^*$ be the optimal path shares solved from Algorithm \ref{alg_overall}. If we directly recommend $p_{hkr}^*$ passengers out of $d_{hk}$ to use path $r \in R_k$, the realized path share will not be $p_{hkr}^*$ due to the behavior uncertainty (i.e., some passengers may not follow the recommendation). Hence, our goal for recommendation strategy is to design an actual path recommendation fraction, $s_{hkr}$, such that the realized path share is $p_{hkr}^*$. 

% Consider a passenger $i$ with OD pair $k$ and departure time $h$. Let $C_i$ be his/her final choice of path and $\tilde{C}_i$ be his/her intended choice of path without recommendation. And let $W_i$ be his/her received path recommendation. We also define $\mathbbm{1}_{\{F_{i,r}|\tilde{C}_i = {r'}\}}$ as an indicator variable for whether passenger $i$ will follow the recommendation or not if he/she is recommended with path $r$ and his/her original path is $r$. Let  $\mathbbm{1}_{\{A_i\}}$ indicates whether he/she is an accessible passenger (i.e., being able to use the recommendation system or not). Then, the random variable that whether he/she will finally use path $r$ can be expressed as

% 
% \begin{align}
% \mathbbm{1}_{\{C_i = r\}} &= \underbrace{(1-\mathbbm{1}_{\{A_i\}})\cdot \mathbbm{1}_{\{\tilde{C}_i = r\}}}_{\text{Condition 1}} + \underbrace{\mathbbm{1}_{\{A_i\}}\cdot \mathbbm{1}_{\{\tilde{C}_i = r\}}\cdot  \sum_{r'\in R_k \setminus \{r\}}\mathbbm{1}_{\{{W}_i = r' \}}\cdot(1-\mathbbm{1}_{\{F_{i,r'} |\tilde{C}_i = r\}})}_{\text{Condition 2}} + \underbrace{\mathbbm{1}_{\{A_i\}}\cdot \mathbbm{1}_{\{\tilde{C}_i = r\}}\cdot \mathbbm{1}_{\{{W}_i = r\}}}_{\text{Condition 3}} \notag \\
% &+ \underbrace{\mathbbm{1}_{\{A_i\}}\cdot \sum_{r'\in R_k \setminus \{r\}}\mathbbm{1}_{\{\tilde{C}_i = r'\}}\cdot \mathbbm{1}_{\{{W}_i = r\}} \cdot \mathbbm{1}_{\{F_{i,r} |\tilde{C}_i = r'\}} }_{\text{Condition 4}}
% \label{eq_condition}
% \end{align}
% Eq. \ref{eq_condition} describes four mutually exclusive conditions that passenger $i$ may finally use path $r$. The first condition means that the passenger does not use the recommendation system but his original choice is path $r$. The second condition means that the passenger uses the recommendation system, has original path $r$, gets the recommendation of using path $r' \neq r$, but does not follow the recommendation. The third condition means he/she uses the recommendation system, has original path $r$, and gets the recommendation not to use path $r$ (then he/she will use path $r$ no matter following the recommendation or not). And the fourth condition indicates the passenger $i$ uses the recommendation system, has the original choice of path $r' \neq r$, gets the recommendation to use $r$, and follows the recommendation.

% By definition, we have $\mathbb{E}[\mathbbm{1}_{\{A_i\}}] = \mu^{\text{A}}_{hk}$,  $\mathbb{E}[\mathbbm{1}_{\{\tilde{C}_i = r\}}] = \bar{q}_{hkr}$,  $\mathbb{E}[\mathbbm{1}_{\{{W}_i = r\}}] = {s}_{hkr}$,  $\mathbb{E}[\mathbbm{1}_{\{{F}_{i,r'}|\tilde{C}_i = r\}}] = {\alpha}_{hkr',r}$, and all indicator variables are independent. As we assume all passengers with the same OD pair and departure time are homogeneous (because we do not have individual level passenger information), $\mathbb{E}[\mathbbm{1}_{\{C_i = r\}}]$ can be seen as the final proportion of passengers in demand $d_{hk}$ using path $r$. It can be calculated as 

% 
% \begin{align}
%     \mathbb{E}[\mathbbm{1}_{\{C_i = r\}}] &= \mu_{hk}^\text{U} \cdot \bar{q}_{hkr} + \mu_{hk}^\text{A} \cdot \bar{q}_{hkr}\sum_{r'\in R_k \setminus \{r\}}s_{hkr'} \cdot (1-\alpha_{hkr',r}) +  \mu_{hk}^\text{A} \cdot \bar{q}_{hkr} \cdot s_{hkr} \notag \\
%     &+  \mu_{hk}^\text{A}\sum_{r'\in R_k \setminus \{r\}} \bar{q}_{hkr'} \cdot s_{hkr} \cdot \alpha_{hkr,r'}
% \end{align}

% Hence, to realize the optimal path share $p_{hkr}^*$, we need to set $p_{hkr}^* = \mathbb{E}[\mathbbm{1}_{\{C_i = r\}}]$ for all $r \in R_k$ and solve for $s_{hkr}$. This provides $|R_k|$ independent linear equations and  $|R_k|$ unknown variables. And it can be easily verified that the solved $s_{hkr}$ satisfying $\sum_{r\in R_k} s_{hkr}= 1$. And the solved $s_{hkr}$ is the final recommended proportion of passengers for using path $r$. 
